What if we have Meta GPT? From Content Singularity to Human-Metaverse Interaction in AIGC Era

The global metaverse development is facing a "cooldown moment", while the academia and industry attention moves drastically from the Metaverse to AI Generated Content (AIGC) in 2023. Nonetheless, the current discussion rarely considers the connection between AIGCs and the Metaverse. We can imagine the Metaverse, i.e., immersive cyberspace, is the black void of space, and AIGCs can simultaneously offer content and facilitate diverse user needs. As such, this article argues that AIGCs can be a vital technological enabler for the Metaverse. The article first provides a retrospect of the major pitfall of the metaverse applications in 2022. Second, we discuss from a user-centric perspective how the metaverse development will accelerate with AIGCs. Next, the article conjectures future scenarios concatenating the Metaverse and AIGCs. Accordingly, we advocate for an AI-Generated Metaverse (AIGM) framework for energizing the creation of metaverse content in the AIGC era.

==> sections/architecture.tex <==
\section{XROS Architecture}

Given the requirements presented in the previous sections and the limitations of existing OSes, we present a novel architecture for an XROS that considers the primary modules of the XR pipeline as resources to be shared between applications.


% By considering the primary modules of the XR pipeline as resources to be shared between applications, an XROS presents an architecture that facilitates such requirements and better integrates XR applications. In this section, we first list XR application requirements before detailing the architecture of the XROS.




\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.6\textwidth}
\centering
\includegraphics[width=\textwidth]{figs/architecture.pdf}
\caption{Potential architecture of an XROS.}
\label{fig:archi}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.39\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{figs/components.pdf}
\caption{Data flows between XROS's modules. }
\label{fig:flows}
\end{subfigure}
\caption{XROS Architecture.  Data from sensors is preprocessed by specialised chips and filtered by the privacy protection module on top of the kernel before reaching the main modules of the XROS. These blocks provide the primitives for XR application}
\end{figure*}


An XROS satisfies the requirements of XR applications by (1) reducing the intermediary layers between sensor data and XR processing, (2)  managing the execution timing of XR operations, and (3) sharing the physical-digital world model among users and applications. The XROS moves from the current interruption-driven task execution model to a steady-state system that periodically processes sensor data. 

\tristan{Most OSes currently used for XR rely on monolithic architectures based on well-established OSes, whether GNU/Linux, BSD, or Windows. Such a choice allows for faster development by relying on a continually updated codebase. Besides, hardware manufacturers develop drivers specifically for these OSes, simplifying the task of integrating new hardware with the OS. The simplicity of development and the readily available drivers compensate for monolithic architectures' disadvantages by allowing developers to focus on the XR operations. We propose that our general architecture be based on an open-source OS such as GNU/Linux. For these reasons, the OS should also be open-source, maximising the possibility of deployment on new devices.}


Our architecture revolves around six primary components presented in Figure~\ref{fig:archi}. \tristan{These components would be implemented as kernel modules to provide better performance and reusability. Such an architecture is inspired by the ROS  architecture\footnote{\url{http://design.ros2.org/articles/ros_middleware_interface.html}}, with the addition of XR-specific and distributed components. }
% This architecture revolves around six primary components that enable a coherent 
% We propose an architecture for the XROS that relies on the six primary components shown on Figure~\ref{fig:archi}. These components interoperate towards performing XR operations within the performance requirements, exposing XR primitives to applications, sharing resources, and providing homogenised interaction and display methods within the XR environment. 

\textit{Environment Understanding:} XR applications build a representation of the users' surroundings.
%The core difference between XR and traditional applications lies on the pervasive sensing of the environment to build a representation of the user's physical surroundings. 
Integrating such techniques at the OS level would improve performance  %enable XR in other OS modules, 
% share the physical world's model among services and applications, 
and provide standardised services to applications. Sharing a single digital-physical world model among applications enables multitasking and shared interaction techniques, improving the system's usability.

% and allows the usage of common visualisation and interaction techniques blended 

\textit{Specialised Chips Drivers:} Scene understanding relies on computation-heavy algorithms. % Many chips enable faster processing, from specialised chips to general-purpose elements such as tensor processing units. 
On-chip asynchronous execution of object recognition, mapping, and localisation would relieve the primary computing units for XR applications. An XROS should leverage these chips to accelerate %the execution of core elements of 
the XR pipeline and improve system stability.

\textit{Network:} Despite specialised hardware, some operations remain too computation-intensive for mobile devices and should be offloaded to more powerful remote servers. %devices at the edge or in the cloud. 
Shared or persistent experiences require combining multiple individual perceptions of the environment towards a single global view. Reliable ultra-low latency transmission of large content is necessary to provide a seamless user experience and prevent decorrelating concurrent user experiences.

%Both operations require methods to compensate for the added network latency

\textit{User Interaction:} A tight integration between Environment Understanding and User Interaction would enable novel interaction methods using the physical-digital duality of XR. Users may leverage the physical world to interact with digital content. %, whether embodied (e.g., gestures) or external (e.g., tangible interfaces).
Integrating interaction at the OS level would also standardise interaction techniques akin to the keyboard and mouse on desktop computers.

\textit{Display:} Display can also benefit from the OS's Environment Understanding to blend digital content with the physical world while avoiding obstruction of critical physical objects or information overload in cluttered areas. 
Multitasking can be enabled by letting multiple applications display content without disturbing each other.

\textit{Privacy:} The XR pervasive sensing process collects massive amounts of personal data on the users and bystanders. Most are irrelevant for applications and can lead to significant ethical and legal issues. The XROS should minimise data between the sensor and the application, network, and display to minimise privacy leakage.


%A layer of privacy protection should minimise data between the sensors output and the other components' input and filter out data for network transmission and display. As such, only manageable amounts of private data would reach the applications.

%Similar to mobile OSes based on UNIX, the remaining parts of the XROS (file system, process and memory management, networking) can be provided by open source components.

These components intercommunicate to reinforce the integration of content with the physical-digital world, as shown in Figure~\ref{fig:flows}. The Environment Understanding module offloads computation-heavy operations through the Network module, compensating latency with the User Interaction module. The User Interaction module leverages the output of the Environment Understanding module to provide interaction methods coherent with the user's physical environment. It also prepares the content for visualisation with the world model in the Display module. 

%\tristan{In the following sections, we detail the operation of each module.}

==> sections/background.tex <==
\section{Background}

XR applications have stringent requirements that are difficult to achieve with current system architectures. This section details such requirements before  highlights current architectures' limitations.

\subsection{Requirements}
\label{sec:requirements}

XR applications superimpose digital content over the users' perception of the physical world. Their requirements are on par with the resolution of the users' perceptive system. Typical guidelines cite a guaranteed minimum of \textit{60\,FPS, with 2k to 4K resolution, and a motion-to-photon latency below 20\,ms} for seamless XR experiences~\cite{8700215}. Such requirements are critical to prevent discrepancies between the user's perception of the physical world and the digital content. \tristan{XR is generally executed on mobile devices. Computation power, storage, network access, and energy consumption are critical. Most operations should execute on-device within the inter-frame time (33\,ms at 30\,FPS or 16\,ms at 60\,FPS)~\cite{braud2017future}. XR applications relying on large environment models should balance the limited device storage space (~10-100GB) and querying remote point clouds of considerable size (several GB for a 100x20m indoor map) through highly variable mobile networks. Finally, with XR running primarily on mobile devices, the system should offer several hours of operations on a full battery charge. XR as a ubiquitous technology also requires to \textit{share the physical-digital world model} between applications and users for simultaneous interaction and multitasking. }

%It thus makes sense for the model to be handled by the OS as a shared resource between applications and devise user interaction methods coherent with such model.

\tristan{\subsection{Current OSes supporting XR}}

\tristan{At the time of writing this paper, XR applications are executed on three type of devices: standalone headsets (Microsoft Hololens\footnote{\url{https://docs.microsoft.com/en-us/hololens/hololens2-hardware}}, Oculus Quest\footnote{\url{https://developer.oculus.com/blog/introducing-oculus-quest-2-the-next-generation-of-all-in-one-vr/}}), mobile phones (Android\footnote{\url{https://developers.google.com/ar}}, iOS\footnote{\url{https://developer.apple.com/augmented-reality/}}, HarmonyOS\footnote{\url{https://developer.huawei.com/consumer/en/hms/huawei-arengine/}}), and headsets offloaded to a powerful local machine (most current VR headsets, e.g., HTC Vive\footnote{\url{https://www.vive.com}}). These devices all feature traditional Windows- or Unix- (Android, GNU/Linux, iOS) based OSes with a monolithic kernel supplemented with user-space modules.} 

\tristan{Many of these OSes execute applications in a compartmentalised fashion for security purposes. For instance, Android creates a new instance of the Android Runtime for each application. XR operations have to be performed for each application independently, causing crippling increases in computation, memory, and energy consumption. Another significant limitation is the lack of networked operation. Most frameworks only consider single-operation networked execution, such as registration in an existing map, and do not fully exploit current and future mobile networks. Fully-offloaded VR headsets act as remote displays, with a single hop to the computing resources. Finally, all existing architectures focus on monolithic kernels, which forces the execution of XR operations further in the user space for stability purposes, impeding performance and flexibility. Microkernels and hybrid architectures could be more adapted to the client-side, while unikernels~\cite{10.1145/3317550.3321445} would considerably enhance performance and security on the server-side. }

\tristan{\textit{Robot OSes}: many robotic applications rely on the same environment understanding algorithms as XR. 
Microkernels have been explored in robot OSes, where each environment understanding operation runs as a separate service~\cite{quigley2009ros}.
However, such an architecture complicates the development and deployment of consumer-grade applications due to limited driver availability, an issue that is less prevalent in robotics. Some Robot OS architectures also provide middlewares for  robot-specific operations on top of existing OSes (e.g., ROS\footnote{\url{https://docs.ros.org/en/galactic/index.html}}), but do not consider user interaction.}

\tristan{In this article, we propose an XROS that addresses the issues of current OSes through a distributed architecture to enable the next generation of XR applications.}


==> sections/cv.tex <==
\section{Environment Understanding}

XR relies on pervasive environment sensing to %build a digital model of the physical world. This model serves to 
 blend digital content with the physical world. In this section, we focus on visual environment understanding, reinforced by information from other sensors (depth cameras, LiDar). %~\cite{campos2021orb}. %To power XR applications and other OS modules, the environment understanding module should provide the base XR primitives and share the access to the world model. 

\textbf{1. XR Primitives.} An XROS should provide XR primitives to applications and services. Current AR frameworks such as ARCore\footnote{\url{https://developers.google.com/ar}} or ARKit\footnote{\url{https://developer.apple.com/augmented-reality/}} %give insights into what components could integrate the OS-level. These frameworks 
combine sensor data to calculate and expose the 3D world model. They provide functions such as plane identification, anchor recognition, and the possibility to save or share the experience. None of these frameworks discloses how the feature points are identified, making the development of additional recognition and segmentation algorithms redundant. 
% An XROS should explicitly expose the feature points extracted from the camera frames and how these points are refined through other sensors. 
The XROS would perform feature extraction and tracking and expose the results to the application. World building and object recognition can be implemented as standardised services to prevent redundancy and improve performance in a highly fragmented market. 
%Providing these functions at the OS level would significantly improve performance by requiring a single execution for all applications. It would also standardise access to these functions in a highly fragmented market. 
Integrating more functions at the lower layers of the architecture would simplify application development, allowing developers to focus on content creation. 
\tristan{Such operation can only succeed in an open-source context to focus the development effort and enable external actors to develop  extensions tailor-made to their usage.}
% Feature extraction and tracking would integrate the kernel to improve performance and expose the calculated feature points to every pipeline layer, while world building and object recognition could be implemented as modules that function as standardised services.


\textbf{2. Shared Access to the world's model.} OSes control the shared access to software and hardware resources for applications. In XR, feature points, world models, semantic areas, and recognised objects are such resources. With a single digital-physical world model to share between applications, the OS decides which application may display content over each area of the physical world, 
% ~\cite{schmalstieg2002studierstube}, 
\tristan{avoiding race conditions, digital asset overlap, visual clutter, and information overload.}
% Such a task involves sharing the physical-digital world in-between applications and deciding which areas from the physical world may not be overlaid with content. 
The OS may define contextual rules based on user safety, information density and visibility, or other cues driven by the user's habits. Leveraging a single world model across applications allows envisioning a more coherent set of interaction methods. 
% Given that all applications use the same environment, it is more natural for users to interact with multiple applications through a similar set of standard interactions techniques.
By combining content visualisation awareness and standard interaction techniques, an XROS can perform more adequate  scheduling, prioritising applications that require immediate display or feedback, similar to how mobile OSes prioritise the application on display. 

\textbf{3. Environment Understanding in Networked Scenarios.} With the recent trend of the metaverse, we expect XR users to share their experiences in real time in a persistent digital world. 
Therefore, many environment understanding techniques may be performed on a powerful server \tristan{or distributed among users} to establish a global model of the physical world. \tristan{Robot OSes provide primitive for collaborative map building. However, XR presents more stringent constraints that prevent their application.} These constraints require keeping a local copy of a simplified environment model to remain on-device for local tracking. Devices may preprocess the sensor data to establish such a local model before transmitting them to update the global world model. \tristan{Computation caching may also accelerate typical operations.} Finally, the local model may also enable OS-level latency compensation techniques that leverage characteristics of the physical world to hide latency from the user (e.g., adapting the geometry of the content to minimise interaction errors caused by latency).

\textbf{4. Specialised Hardware.} Integrating complex image and sensor processing operations in the OS may significantly impact the system's operation. Some operations are computation-heavy, while others rely on manipulating large data structures, monopolising the device's resources. %Many of such operations may occupy the entirety of the computing resources for a significant duration. %, preventing the rest of the pipeline to be executed. 
With the XR pipeline requiring a steady-state operation, computation-heavy operations must be executed in a non-blocking fashion.
Besides, many of these operations may be prone to errors caused by unexpected input \tristan{which may be disastrous at kernel level}. %If implemented at a low level in the architecture, 
%As such, integrating all operations in the kernel may be counter-productive. 
Specialised hardware may handle repetitive operations more efficiently. We consider three types of hardware: (1) highly specific single-operation chips for data preprocessing (feature extraction), %~\cite{nikolic2014synchronized}, 
(2) specialised hardware tapping into the memory of the processor to perform more complex operations (mapping, object recognition), %~\cite{nguyen2019high}, 
and (3) more general chips (rendering, machine learning). Nowadays, most mobile devices embed chips belonging to the third category, but many works study FPGAs for computer vision. The XROS should leverage such chips to relieve the load and minimise the impact of errors.

==> sections/evaluation.tex <==
\section{\added{Illustration}}

\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figs/appA.jpeg}
    \caption{App A}
        \label{fig:appa}
    \end{subfigure}
    \begin{subfigure}[t]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figs/appB.jpeg}
    \caption{App B}
            \label{fig:appb}
    \end{subfigure}
        \begin{subfigure}[t]{0.22\textwidth}
        \includegraphics[width=\textwidth]{figs/appAB1.jpeg}
    \caption{App A and B - Shared world model}
            \label{fig:appab1}
    \end{subfigure}
        \begin{subfigure}[t]{0.22\textwidth}
                \includegraphics[width=\textwidth]{figs/appAB2.jpeg}
    \caption{App A and B - Parallel execution}
            \label{fig:appab2}
    \end{subfigure}
    \caption{\added{Operation considered: (a) and (b) isolated execution; (c) Shared environment model, button-operated context switching; (d) Parallel execution, shared world model}}
    \label{fig:app}
\end{figure*}


\added{To illustrate the need for a shared world model, we implement an application that anchors an object to a detected plane by tapping. We implement the application on Android with ARCore, through Unity's ARFoundation. We compile two versions: app A spawning a red cube, app B spawning a blue sphere (Fig.~\ref{fig:appa} and~\ref{fig:appb}). Due to Android's architecture, each application builds an isolated world model with a single application running at a given time. }

\added{We initialise app A and B, start app A, switch to app B, and back to app A. We measure the time for tracking to recover when app A regains focus. We first consider the device fixed in a static position. Over 10 measurements, tracking recovers in \textit{1.35\,s} on average (stdev = 0.29\,s), accounting for a large share of the context switching. We then consider the device moving so that app A regains focus in a different location. We conduct the experiment in a 13.5\,sqm office.
When app A's red cube location remains in the camera view, tracking recovers in an average of \textit{1.53\,s} (stdev = 0.49\,s). 
When the device's camera points away from the red cube or the motion is too significant, the user must move the smartphone to regain tracking, adding a minimum of\textit{3\,s}.}
%However, when the device's camera points to a direction that does not contain the red cube or motion is too big, the user often needs to further move the smartphone for the tracking to recover, adding a minimum of\textit{3\,s}.


\added{We then consider an application implementing app A and B over a single world model, with button-operated context switching (Fig.~\ref{fig:appab1}). As the applications are lightweight, objects are destroyed and reinstantiated within the interframe time (\textit{16\,ms} at 60\,FPS). Sharing a single world model between applications thus results in 99\% shorter tracking recovery times, with no tracking loss. We finally implement a version of the application where both applications run at the same time with separation between applications based on the location of the content (Fig.~\ref{fig:appab2}). In this case, we remove the need for context switching, as both apps are running at all times, simplifying multitasking.}

==> sections/implementation.tex <==
\section{Concluding Notes, Discussion and Implementation}

%This article proposes a modular architecture for an XROS centred around the environment understanding module that builds a digital representation of the physical world. This world model drives user interaction and content visualisation at the system level and exposes XR primitives to applications. Besides noticeable performance improvements, integrating the world model at the OS level unlocks new functionalities for pervasive XR, including multitasking, reduction of information overload, standardisation of interaction methods, and large-scale multi-users and persistent experiences. Integrating complex operations at the lower layers of the system comes with significant implementation challenges, as follows:
This article details the architecture of DiOS, an XROS architecture that addresses the stringent requirements of pervasive multi-user XR, enabling exciting developments such as the metaverse.
We offer a modular design for an XROS centred on environment understanding. The world model drives system-level user interaction and content visualisation and provides XR primitives to apps. 
Integrating the world model at the OS level enables additional functions for ubiquitous XR, including multitasking, standardised interaction techniques, and large-scale multi-users and permanent experiences. Complex processes at lower system levels provide considerable implementation issues, and hence implementation challenges, as follows.

\textbf{1. Stability.} Most OSes deploy several layers of abstraction between the kernel and the application. This type of architecture ensures fairness in accessing system resources and prevents bugs from affecting the entire system. Integrating XR operations at the lower levels thus requires the utmost care. XR data processing relies on complex algorithms, which stability is difficult to assess. Errors may significantly affect the operation of the entire OS. %Minimising the impact of such errors can be done both at the hardware and software levels. 
Running XR operations on specialised chips would delegate operations to physically separated hardware but is less flexible. In software, some operations (e.g., feature extraction) could be executed at the kernel level, as their timely execution is essential. More sophisticated operations may be implemented in the user space, letting the process schedulers handle access to resources and minimising the impact of errors. %, thus preventing them from using more resources than necessary while minimising the impact of errors.

\textbf{2. Network.} Network access is essential to offload computation-heavy operations and retrieve shared or persistent elements. Such a model disrupts the status quo of traditional self-contained OSes. With the emergence of massive multi-user persistent experiences such as Facebook's metaverse or Niantic's planet-scale AR project, distributing OS-level operations would enable better integration of remote content. The XROS architecture could become completely distributed, leveraging remote sensors and computation resources dynamically. % depending on the state of the system, the local user context, and the task to execute.
\ahmad{3GPP \footnote{\url{https://www.3gpp.org/news-events/2152-edge_sa6}} 
provides native support for edge computing, including application layer architecture and media processing. The application architecture comprises the Edge Enabler Server, primarily responsible for enabling the discovery of the Edge Application Services; Edge Enabler Client, providing support functions such as the discovery of Edge Application Service in the client device (e.g., VR Headset, mobile-phone). Including Edge Enabler Client as a component in XROS would enable the automated discovery of edge services.} %Afterwards, the Offloading Manager can offload the task to the remote server based on parameters determined by the Profiler (see Figure~\ref{fig:network-offload}). These parameters are classified into five categories, 1) Network Specifications: the network type such as 3G, LTE, WiFi and 5G, the available bandwidth and latency, 2) Mobile Specifications: CPU speed, battery level, and available Storage and memory, 3) User Preferences: privacy and data confidentiality, 4) Task Specifications: execution time, and 5) Server Specifications: CPU speed, available storage and memory, and load. }

\textbf{3. Interaction in XROS.} %Back in the days when we only had archetypical operating systems, application developers on 2D UIs had to manage some control programs for I/O devices. 
%The modern operating systems read from and write to I/O devices, including printers, mouse and keyboard duos, and displays. Remarkably, input and output operations represent significant proportions of instructions (i.e., I/O commands) in modern operating systems. For example, moving a mouse cursor continuously from one corner to another. 
%XR environments go beyond the 2D UIs in our traditional desktop interfaces. By integrating physical elements into the digital world, blended UIs can leverage the physical world model to provide more intuitive visualisation and interaction. However, standard interactions are essential to such intuitiveness. Ideally, the XROS should enable typical interaction methods across all applications, on top of which individual programs may integrate specific operations. %For instance, gestures for grabbing a virtual object, pressing a button, resizing a component should be defined system-wide.
%The application may define other gestures, such as throwing a ball in a video game.
Modern operating systems read and write to printers, mouse-and-keyboard duos, and displays. Input and output operations form a large fraction of operating system instructions (I/O commands), e.g., moving a mouse pointer from one corner to another.
XR environments surpass 2D desktop UIs. Blended UIs can provide more intuitive visualisation and interaction by integrating physical elements into the digital world. Standard interactions are key to intuitiveness. XROS should enable standard interaction methods across all applications, on top of which programs can add specific operations. 

\textbf{4. Scheduling and Shared Resources.} OSes share hardware and software resources among applications. We consider the physical-digital world model as a shared resource at the core of the XROS. Applications need to request access to the world model to read (access XR primitives) and write (overlay content). The OS keeps track of where applications display content to avoid overlapping content and minimise information overload for the user. %The process scheduler can prioritise applications displaying content in the user's current field of view. It may also favour the pre-computation of heavy operations for applications which content is located in the vicinity of the user yet hidden from the users' view and handle other applications with low priority.
The process scheduler prioritises apps displaying content in the user's field of view. It may also pre-compute heavy operations for apps whose content is near the user but concealed from view and handle other applications with low priority.

\tristan{\textbf{5. Energy Consumption.} 
XR is employed in mobility and relies on computation-heavy algorithms, hence energy consumption impacts design and implementation. Each module should be designed to minimise energy use, e.g., monolithic kernels. %As most modules have limited downtime, we reduce communication between modules and applications to save energy. %With XR being primarily used in mobility while relying on computation-heavy algorithms, energy consumption affects every step of the design and implementation. Similar to privacy, each module should minimise energy consumption by design. Energy consumption is also one of the reasons for using a monolithic kernel approach. 
As most modules will run periodically with little downtime, we minimise the energy consumption by reducing communication between modules and between modules and applications.
}
The XROS may be readily implemented using current resources and a modified Linux Kernel to handle computer vision operations and I/O scheduling. The remaining operations may be done in user space using GNU tools. The privacy module would be implemented between kernel pre-processing and user space operations.
%Implementing such a system can be easily performed over existing resources, leveraging a modified version of the Linux Kernel to handle primary computer vision operations and build a world model for application and I/O scheduling. The remaining operations can be implemented in user space, supported by the traditional GNU tools. The privacy module's implementation would occur between the kernel pre-processing of the sensor data and the actual interpretation in user space. 

==> sections/interaction.tex <==
\section{Novel Interactivity with XROS}\label{sec:user-inputs}



% The XROS aims to deliver users a new reality that perfectly blends the real and digital worlds. As such, it may no longer be centered around a desktop displaying windows. %Thus, user interactivity of AROS has to be designed from a user-centric perspective.
% \textit{Reality-Based Interaction} (RBI) describes the user's desire towards the realism of interfacing objects and daily practices belonging to the non-digital world. 
% ~\cite{RBI-CHI08}.
Interaction techniques in OSes can have significant effect on how users gain ownership of the system~\cite{10.1145/3334480.3382944}.
The XROS goes beyond the 2D user interfaces (UIs) and emphasizes the interactivity with users' physical bodies, surroundings, and other users~\cite{RBI-CHI08} 
%In addition, our physical urban environments will look completely different as increasing immersive contents blended into our urban environments~\cite{csur-lee-hcityI}.
 as follows: %the requirements of user interactivity with AROS can be categorized into four aspects.

\textbf{1. Blended UIs in the physical world.} 
%the development of AR - single, 
% The definition of augmented reality has been evolving from overlaying simple information to blended environments combining physical and digital seamlessly~\cite{MR-def-CHI19-Speicher}. 
Novel UIs across the digital and physical worlds can serve numerous users to experience high immersion and virtuality in heterogeneous environments (Figure~\ref{fig:ego-act}). The XROS should facilitate multiple users to collaborate with such virtual interfaces superimposed on the physical world. These blended UIs should be ubiquitous, potentially up to city-scale~\cite{csur-lee-hcityI}. \tristan{Achieving city-scale XR would need interdisciplinary efforts between urban designers, telecom operators, and computer scientists,} driven by a  \textit{distributed XROS} with \textit{advanced mobile networks} to synchronise multitudinous objects and their corresponding blended UIs. 

% A recent focus group interview with ten experts of virtual environments reveals that augmented reality is evolving~\cite{MR-def-CHI19-Speicher} from overlaying simple information (e.g., the first prototype of AR named The Touring Machine~\cite{Feiner1997ATM}) to handling contents more enriched than ever before~\cite{ssin2021udt}. 
% As such, the experts generate working definitions for a stronger version of augmented reality -- a blended environment, as a novel UIs across digital and physical realities, can serve numerous users to experience high levels of immersion and virtuality, in heterogeneous environments. 
% In other words, the AROS should own the capacity of facilitating multiple users to collaboratively work with such virtual interfaces superimposing on the physical world.
% Additional, it is necessary to build the AROS that enables users to interact with the blended UIs ubiquitously, perhaps everywhere and anytime on a city-wide scale~\cite{csur-lee-hcityI}. The challenges of achieving the city-wide requirements would need interdisciplinary research efforts, primarily driven by \textit{distributed AROS} with \textit{advanced mobile network} to synchronize multitudinous everyday objects and their corresponding blended UIs (i.e., \textit{extended reality}). 


%physical 
%everywhere

%mobile

 \begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/ego-3.JPG}
    \caption{Virtual-Physical User Interaction in XROS\protect\footnotemark.}
    \label{fig:ego-act}
\end{figure}
    \footnotetext{Images from the Ego4D dataset samples \url{https://ego4d-data.org/fig1.html}}

\textbf{2. Enhanced Awareness to Users and Their Environments.} 
To achieve blended UIs, the digital overlays should match with objects, locations and people in the physical world. %~\cite{KAIST-woo-context-awareness}. 
The XROS uses context awareness to understand the user's situated environment. %~\cite{cloud-or-not-cloud}. 
%The XROS can achieve context awareness 
The XROS may recognize visual markers or 3D features on physical objects and users' body gestures~\cite{edgexar}. 
% ~\cite{Hariharan2015HypercolumnsFO}. 
However, such recognition requires significant computational resources. Similar to the X windows system\footnote{https://x.org/wiki/}, the XROS may consider thin clients to display the overlay while UI operations are performed on a separate machine. %Therefore, Task offloading techniques serve to alleviate the bottleneck on AR devices but maintain low latency for the sake of responsive user interaction~\cite{Zhang2018JaguarLL} and realism~\cite{louis2019real}.

\textbf{3. Mobile User Interactivity.} 
The XROS provides users with the fundamental input and output (I/O) functions. Users receive enriched AR information, whether visual, audio, or haptic. 
% ~\cite{10.1145/3457141}). 
The critical bottleneck of XR displays is the user's cognitive load. Displaying content without proper selection and management would cause information overflow and poor usability~\cite{Lindlbauer2019ContextAwareOA}.
%It is important to note that another key bottleneck of AR display is the user's cognitive load. That is, displaying Ar contents without proper selection and management would cost users to drop the XROS due to information overflow and  poor usability~\cite{Lindlbauer2019ContextAwareOA}. 
Thus, the XROS has to maintain highly relevant content inside the size-limited lens of XR~\cite{A2W-kityung}. %~\cite{Lee2020FromST}.
The XROS should also adapt to the vastly diversified input interfaces, whether embodied or physical.

% mobile input techniques, including voice commands, miniature wearable devices, on-body and on-skin interfaces, the surface of everyday objects~\cite{csur-lee-hcityI,u258}, to make responses with displayed AR contents. The AROS should adapt to such vastly diversified input interfaces.

\textbf{4. Towards Tangible Interaction} As a final note, the blended UIs of the XROS do not limit to physical-digital mixed overlays. Tangible interaction will redefine our spatial environments. 
Remarkable examples of tangible interaction include public displays, interactive tabletops, mechanised infrastructures, at-home IoT devices, drones, augmented surface of electronics~\cite{shaer2010tangible}. %Remarkable examples of tangible interaction include movable public displays~\cite{10.1145/2559206.2579410}, interactive tabletops~\cite{tabletop-AR}, mechanised infrastructures~\cite{robot-architecture}, at-home IoT devices~\cite{michalakis2018visualizing, cao2019v}, drones~\cite{Yau2020HowSC, flying-lego-brick}, augmented surface of electronics~\cite{freeman2014tactile}. 
Thus, \textit{how to manage countless distinct tangible items} remains a critical challenge. 
% AR-IoT Interaction

\textbf{5. I/O under the XROS perspective} The physical world, a non-static environment, is characterized by highly diversified events and dynamic situations. When we move the blended UIs in an OS serving virtual-physical environments, \textit{Personal Space Distance} can consider various items and animate characters in users' surroundings, acting either `to-be-augmented' (Output) or `\textit{clickable}' (Input). For instance, our bodies in an intimate zone, objects in a personal zone, and bystanders in the social distance can become I/O candidates for blended UIs. 

%The existing frameworks supporting XR do not serve the purpose of understanding items and animating characters in our physical worlds. Such frameworks encourage developers to establish I/O events with a limited number of physical objects. Such I/O events are often distinct from other applications. Instead, a holistic view supported by XROS supports a comprehensive understanding of the world model, characterized by spatiality, time/chronology, semantics and ontology. %Although we have no definitive answers to manage the factors for blended UIs, 
%The world model under the governance of XROS will streamline I/O and sensors to achieve enhanced awareness of users' situations and smart localization of interactivity candidates among augmented objects. 
% Without an OS to handle I/O events in virtual-physical environments, XR will be hindered by scalability issues and development efforts.

Existing XR frameworks don't grasp tangible goods or animate characters. Such frameworks encourage developers to create less I/O events. I/O events are typically unique to apps. XROS enables a holistic view of the world model, which includes spatiality, time/chronology, semantics, and ontology. 
The XROS-governed environment model will simplify I/O and sensors to improve user awareness and localise interaction candidates among augmented items. 
XR will have scalability and development challenges without an OS to manage I/O in virtual-physical settings.

%blended UIs of virtual-physical environments lead to higher uncertainty than the UIs on traditional OS. That is, 

%Static interfaces - no 
% everythings can be interfaces in blended UIs and tangible interaction
% I/O no longer limits to a 



==> sections/network.tex <==
\section{Networking}

 \begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/network_offload.pdf}
    \caption{Task offloading primitives.}
    \label{fig:network-offload}
\end{figure}

The previous section raised the need for on-device scene understanding. Remote scene understanding is critical for executing computationally heavy XR operations and supporting persistent or shared experiences. The XROS should thus supplement standalone operation with %data and computational power from 
remote units.



\textbf{1. Computation Offloading.}
The XROS may offload computation-heavy tasks to remote machines. Using background microservices, the XROS can estimate the computational cost of XR operations, maintain connections to servers,  provide handover, and decide when and where to offload tasks. It should also allow developers to specify whether a task is executed on the device or remotely. 
\ahmad{Figure~\ref{fig:network-offload} illustrates multi-tiered computation offloading where computing occurs on servers collocated with base stations or in the cloud. As an essential component in XROS, the Edge Client Enabler enables  handover as the user moves range and ensures the subsequent server migration for uninterrupted XR experience.}
% Figure~\ref{fig:networks} illustrates how computation offloading and handover management could take place in 5G with a 2-tier server architecture. Background microservices detect when the user moves out of the eNodeB's range to the gNodeB,  perform handover, and migrate.

\ahmad{The Offloading Manager decides whether to offload a task based on parameters determined by the Profiler. These parameters are classified into five categories, 1) Network Specifications:  network type (3G, LTE, WiFi, 5G),  available bandwidth, and latency, 2) Mobile Specifications: CPU, battery, storage and memory, 3) User Preferences: privacy and data confidentiality, 4) Task Specifications: execution time, and 5) Server Specifications: CPU, storage and memory, and load. The profiler also drivesAudio video (AV) encoding and decoding, at the interface between the hardware and the OS.}




%  \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{figs/networking.pdf}
%     \caption{Handover and multi-tiers offloading in XROS.}
%     \label{fig:networks}
% \end{figure}



\textbf{2. Shared and Persistent Experiences.} 
One of the most ambitious advances for large-scale XR consists in allowing multiple users to share the same experience spatially and temporally. 
%Two of the most ambitious projects for large-scale XR environments are enabling multi-user experiences and establishing a persistent digital world. 
%One of the main projects for large-scale XR environments is the persistence of the XR world, 
%allowing multiple users to share the same experience at the same location. %Such operation has significant implications in terms of computing and network architecture. 
Such applications aggregate the environment model of multiple devices to build a global model, enabling concurrent interaction with the digital content. The location-awareness of edge servers may perform this aggregation at a computationally acceptable scale. Device-to-device communication enables immediate communication between users. %~\cite{ansari20175g}. 
%The technology required to create multi-user XR applications can also create persistent digital worlds across devices. 
Digital persistence allows users to create or modify digital content in a given physical location and share it with other users through the network.
The XROS will thus face the challenge of relying on external providers to aggregate data, provide computation offloading, and store persistent content.
\ahmad{The Edge Enabler Client allows users in the same vicinity to share experiences by interacting with the same edge server. Handover is guaranteed upon user mobility to another Edge server's range\footnote{\url{https://www.3gpp.org/news-events/2152-edge_sa6}}.}

\textbf{3. Content transmission.}
The XROS will rely on distant servers at the edge or cloud to offload computations and provide shared experiences. XR presents significant bandwidth, latency and reliability constraints.
Latency and bandwidth can be optimised through efficient usage of the available resources~\cite{braud2017future}. %Transmitting data within the latency and reliability constraints of XR is a significant challenge. Besides network latency, 
The transmission may experience packet loss due to core network congestion or channel error in the access network. The XROS should thus monitor the network conditions and dynamically adapt the recovery techniques~\cite{alhilal2022nebula}. Similar to WebRTC, the XROS would obtain a better trade-off between temporal quality (smoothness of rendering), spatial video quality and end-to-end delay by utilising an adaptive hybrid NACK/FEC method~\cite{loss2013webrtc}. The XROS should also adapt the transmission rate to the available bandwidth, either by adopting elements of WebRTC (application protocol) at the transport level or
developing novel transport protocols that integrate adjustable video rates and  mitigate packet loss.

\textbf{4. Latency Compensation.} Although computation offloading enhances the capabilities of constrained hardware, it comes at the cost of network latency. Such latency adds up to the the total motion-to-photon latency (the latency between user motion and its impact on the display), and thus reducing the immersion~\cite{braud2017future}. Latency compensation techniques should be designed to hide such latency from the user. Services may track the features of captured images until object recognition results are received to adjust to the device orientation~\cite{edgexar}. Geometric latency compensation may also provide larger interaction targets in case of increasing motion to photon latency.

\tristan{\textbf{5. Server Architecture.}} 
\tristan{In this article, we primarily focus on the XROS from the client perspective, following a monolithic kernel  to leverage the established codebase and simplify driver integration for new hardware. However, the server-side of the XROS exhibits different requirements, such as stability and performance, while running on standard hardware architectures. As most XROS distributed operations are very specific (registration, multi-user interaction, computation offloading), we propose using unikernels on the server~\cite{10.1145/3317550.3321445}. Such unikernels consist of minimal images that heavily link the application to a specialised kernel, providing better stability, performance, and security by compartmentalising each operation.}

% %Emerging XR-based 3D gaming relies on rich resources (i.e., GPU, TPU, and Huge Memory) to render sophisticated 3D scenes and overlay digital objects.  
% XROS must support computation offloading as a crucial component in the pipeline (user-motion to scene rendering). Using micro background services, XROS estimates frame rendering delay, maintains connections to remote candidate servers (potentially MEC servers) and provides handover on user's coverage change~\cite{tbraud2021talaria}, and decides whether to offload tasks or not. Moreover, 





==> sections/privacy.tex <==
\section{Security and Privacy}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/XOS_privacy.pdf}
    \caption{Privacy protection architecture enforcing privacy on the application's input (sensor data) and output (display, haptic) flows.}
    \label{fig:privacy}
\end{figure}

XR pervasively senses the users' physical surroundings. Therefore, it faces multiple security and privacy challenges~\cite{lebeck2017securing}. OS-level privacy protection mechanisms offer more comprehensive treatment of personal data~\cite{268928}. \carlos{The XROS includes a modular privacy abstraction layer on top of the system's kernel that allows the creation of tailored privacy policies according to the sensor (hardware) and users' privacy profiles~\cite{lefeuvre2021flexos}. This section focuses on the spatial data collection},  on users and bystanders, and consider both the I/O flows (Figure~\ref{fig:privacy}). 

\textbf{1. Spatial Data Collection.} 
% Spatial data has become more ubiquitous with the rising adoption of XR technologies in mobile environments. 
Spatial information allows XR applications to understand the user's surroundings better. 
% and opens new threats to users' and bystanders' privacy. 
%However, such data can be used to infer spaces from the captured 3D point clouds and allow an attacker to recognise space/objects belonging to a specific user despite the lack of visual images~\cite{guzman2021unravelling}. 
Such data may be used to infer spaces from 3D point clouds, allowing an attacker to recognise a user's space/objects without visual imagery~\cite{guzman2021unravelling}.
%An XROS should protect such data against potential threats. The input spatial data sanitation should include user-defined preferences about the level of data collected by sensors and a context-based framework that can (automatically) obfuscate objects and individuals. 
An XROS should safeguard such data. Input spatial data cleaning should contain user-defined options concerning sensor data level and a context-based framework that may hide objects and persons.
% whether an object, face in the field of view should be obfuscated. 
\carlos{%The privacy manager will control how the information is being collected. The technologies to protect users' privacy and their surroundings can be based on fine-grained privacy-enhancing technologies (PETs)~\cite{tavani2001privacy} applied to the respective level of data according to user-defined and context-based policies.
The privacy manager controls data collection. Fine-grained privacy-enhancing technologies (PETs)~\cite{tavani2001privacy} may be used to safeguard users' privacy and surroundings depending on user-defined and context-based regulations.
} 
% For example, a PET can obfuscate only persons in the field-view of the sensors (e.g., persons in the video feed or cloud points).
\balance

\textbf{2. Bystander Privacy.} 
% XR's pervasive sensing may affect the users' privacy. 
% Many legal frameworks require data collection systems to give data subjects control over their personal data~\cite{EUdataregulations2018}. 
As non-users, bystanders often do not have control over their data, which complicates XR's legal and ethical application. An XROS should thus automatically detect and minimise data from bystanders~\cite{shu2018cardea}.
Bystanders don't manage their data, which complicates XR's legal and ethical applicability. The XROS should identify and minimise bystander data.
%Following the above context-based and user-defined policies, the XROS should apply obfuscation techniques to any individual in the sensor range. Moreover, the XROS should include protection mechanisms to communicate privacy policies from bystanders using a seamless approach, e.g., hand gestures~\cite{shu2018cardea} or D2D communication. 
The XROS should apply obfuscate private data in sensor range depending on context and user-defined restrictions while seamlessly conveying privacy preferences and policies (hand gestures, or D2D communication).
The XROS should apply bystanders' input preferences under the same framework as the existing rules.

\textbf{3. Input Data.} The XROS should include an input protection layer as an intermediary framework between raw sensor data and  XR applications. \carlos{The protection layer splits the access control and processing of the sensed data.} 
% ~\cite{hu2021lenscap}.} 
% We build on top of~\cite{hu2021lenscap}, where the protection layer splits the access control and processing of the sensed data. 
%This approach relies on three modules: sensor collection, sensor data, and network manager. Each sensor includes a sensor collection module, where developers can directly access the sensed data on-device. The sensed data is stored in the database module, where applications can access and process the collected data. The network process allows XR applications to share the sensed data with external parties (e.g., cloud computing and multiplayer games). The privacy manager regulates access to data by external parties (applications, remote servers). The privacy manager combines user-defined and OS-defined rules to control the information sharing with third parties via the network module.
Sensor collecting, sensor data, and network management make up this strategy. Developers may easily access sensed data on each sensor's sensor collecting module. Applications may access and handle detected data in the database module. XR apps communicate detected data with other parties (e.g., cloud computing and multiplayer games) through mobile networks. The privacy manager controls external data access (applications, remote servers). It combines user-defined and OS-defined restrictions to regulate network module information sharing.


\textbf{4. Output Data and Safety.} 
%Malicious XR output can raise new privacy threats~\cite{lebeck2017securing}, for instance, occluding physical objects that present a risk for the user. Therefore, the XROS includes a policy manager with well-defined parameterised conditions and actions to perform the XR output.
Malicious XR output may create additional privacy issues by obscuring user-risk items~\cite{lebeck2017securing}. XROS's policy manager contains well-defined, parameterised criteria and actions for XR output. 
In~\cite{lebeck2017securing}, the authors propose an XR platform that controls the output that applications can display according to context-aware policies. 
% The output policies constrain the virtual content users can see in the XR applications.
%The policy manager includes user-defined and context-based policies. The user-defined policies allow the user to filter unnecessary information (e.g., ads). The context-based policies are aware of the user's situation (e.g., less visual information when driving). The XROS policy manager should also handle non-visual outputs such as audio and haptic feedback. 
% and display priority when several applications share the physical world's real estate. 
The policy manager comprises user- and context-defined policies. The user-defined rules filter unwanted information (e.g., ads). The context-based rules know the user's circumstances (e.g., less visual information when driving). The XROS policy manager should handle audio and haptic outputs as well.
Besides safety issues, output data should undergo another layer of minimisation before being displayed or transmitted to remote machines.
 %In addition to safety, output data should be capsuled before being presented or delivered to distant computers.

Privacy and policy managers, while different,  have a similar architecture. 
% , where user and context-based policies will control the data collection and visualisation, respectively. 
%The privacy manager includes privacy protection tools specifically for each of the sensors and techniques (e.g., rules) to avoid the privacy threats of data aggregation from different sensors' data. 
% (e.g., an attacker using an application to collect). 
%The policy manager enforces policies to control the output data layer. 
The privacy manager offers tools to secure each sensor's privacy and approaches (rules) to prevent data aggregation concerns. The policy manager controls the output data layer policies. 
% These constrain-policies can adapt to the device (display, vibroactuator) using context-based rules, such as no haptic feedback while driving a car. 
It also includes an abstraction layer to integrate the different output devices and artefacts (e.g., objects in the field of view) where the XROS can render information. 



% \textbf{}
% In particular, spatial data has become more ubiquitous with the raising adoption of XR technologies in mobile environments~\cite{guzman2021unravelling}. This spatial information allows XR applications to better and more precise understanding of the surroundings. However, this data opens new threats to users' privacy. For example, the spatial data collected by Microsoft HoloLens (used to overlay digital interfaces on the physical world) can be reversed to infer spaces from the captured 3D point cloud. This spatial information can allow an attacker to recognise space/objects belonging to a specific user, despite having any visual images (e.g., photo, frame)~\cite{guzman2021unravelling}.

% %We consider

% XR technologies sense the users' physical surroundings and overlay digital visual, audio, and haptic signals over the real-world view~\cite{roesner2014security}. Therefore, XR can face several privacy challenges according to the technologies used to deliver XR experiences. Following previous works~\cite{roesner2014security,lebeck2017securing,de2019security,guzman2021unravelling,hu2021lenscap} shows the different aspects that XR systems should include to protect users' privacy: \textit{i)} input, \textit{ii)} output, \textit{iii)} data access, and \textit{iv)} interaction. 


% XR applications are characterised by the sensing capabilities of their devices. For example, AR applications will use the camera frames to render the virtual objects on the physical world. VR applications will monitor the hand and head movements to display the virtual view and hand movement accordingly. The continuous sensing opens new privacy risks greater than conventional systems such as desktops~\cite{roesner2014security}. In many cases applications collect more than the required data (geoposition of the user) to render their experience, instead of the relative change in position using accelerometer and gyroscope data.

% XROS also protect users' input interactions such as hand gestures. Sensors that use vision-based natural user interfaces can capture more information than the hand gesture related data. Therefore, XROS includes a module to manage the access of the sensing data by applications, as we will describe later in this section.

% Spatial data has become more ubiquitous with the raising adoption of XR technologies in mobile environments (e.g., Pokemon Go, Oculus)~\cite{guzman2021unravelling}. With new advances in sensor technology, mobile devices can now capture 3D representations (e.g., point cloud, trackable planes) of the physical world. This spatial information allow XR applications to acquire better and more precise understanding of the surroundings. However, this data opens new threats to users' privacy. For example, the spatial data collected by Microsoft HoloLens (use to overlay digital interfaces on the physical world) can be used to infer spaces from the capture 3D point cloud. This spatial information can allow an attacker to recognise space/objects belonging to a specific user, despite having any visual images (e.g., photo, frame)~\cite{guzman2021unravelling}.

% Protection techniques in XR systems focus primarily on the collected visual information by reducing the amount of information collected by RGB cameras. These abstraction approaches (e.g., skeletal representations) focus on protecting traditional visual information such as images and video. Spatial data can contain a simplify representation of user spaces, including objects and individuals (e.g., users, bystanders). Nevertheless, the spatial representation can be used together with novel deep-learning based 3D classifiers such as shape classifiers~\cite{qi2017pointnet++} and generators~\cite{spurek2020hypernetwork}, to enhance the XR experience with 3D spatial information. However, the spatial data protection remains limited in their development.  


% The ubiquity of XR applications provides users with multi-user interactions, sometimes physically co-located (e.g., Pokemon Go). These immersive and multi-user contexts can present several privacy risks for users and bystanders~\cite{lebeck2018towards}. for example, the use of XR applications in public environments can affect bystanders when the devices sense them (e.g., they are in the camera field-of-view). According to the findings in~\cite{lebeck2018towards} users are concerned about the visual captured information that XR applications can collect about users' surroundings. In terms of multi-users XR applications we can observe several challenges~\cite{lebeck2018towards}: access control, which can include how virtual objects are visualised (e.g., not allowing the rendering on top of other users for malicious purposes such as mocking them); ownership of virtual objects; personal space in XR, how XR applications manage the personal space (e.g., control the rendering of virtual objects inside the physical personal space of another user or bystander). 



% Following previous works~\cite{jana2013scanner,hu2021lenscap,guzman2021unravelling}, XROS includes an input protection layer under the privacy module. The protection layer is an intermediary framework between raw sensors data and the XR applications. We build on top of to~\cite{hu2021lenscap}, where the protection layer splits the access control and process of the sensed data (e.g., visual frames). The split-approach consists on three different modules: sensor collection, sensor data, and network manager. Each sensor will include a sensor collection module, where developers can collect and access the sensed data on-device. The sensed data is also stored in a database module, where other modules of the applications (e.g., audio feedback) can access and process the collected data, for example from visual sensor (e.g., camera). The network process will allow the XR applications to share the sensed data with external parties (e.g., cloud computing, multiplayer game) to process heavy computational methods in the cloud. 



% %Data access
% \subsection{Input data}

% The proposed system also includes several data protection techniques in the aforementioned sensor collection and data modules. The first module protects the input data from the sensors using a management framework. This framework allows users to specify and control how the applications access the different sensors' data (similar to Android and iOS permissions). This module also includes privacy-enhancing techniques (differential privacy, k-anonymity) to be applied to the collected data before being stored (for a specific amount of time) in the data module. The data module allows applications to send the protected data via the network module. Other applications can also access the stored data (in multi-application scenarios). The data module also allow developers to aggregate different types of data (from different sensors) using privacy-preserving data aggregation. The aggregated data includes multiple collection or sensor points, such as the 3D scan of a room, while preserving the individual information. Finally, the applications can process the sensed data in the data module using secure multi-party computation and zero-knowledge proof. These protecting processing approaches allows the applications to process the collected information from several sensors without knowing precisely the actual sensed data.

% The network manager includes several permissions (similar to permission access in mobile OS) that are continuously monitored to avoid sharing of unwanted data. Due to the multimodal nature of XR experiences, we include the sensor data module, where the collected data by one sensor (camera frame) can be used to display other data in the users' output (e.g., audio, haptic).

% % Output
% \subsection{Output data}

% Although the privacy risks of XR applications and the input data they collect through different sensors, the malicious XR output in such immersive applications~\cite{lebeck2017securing,roesner2014security} can raise new privacy threats.
% For example, we can imagine an XR-enabled windshield where road and traffic information is overlaid in the driver's view. An attacker can overlay digital artefacts such as text on top of real speed limit signs, putting in risk the driver and other occupants in the vehicle. In~\cite{lebeck2017securing}, the authors propose an XR platform that controls the output that applications can display according to a set of context-aware policies. The output policies constrains the virtual content that users can see iston the XR applications. These policies should be restrict to avoid any challenges and privacy risks that more arbitrary (less restrictive) policies can cause in the XR output. Therefore, XROS includes a policy framework with a set of well-defined parameterised conditions and actions to perform in the XR output. For example, when a particular condition is true (e.g., object is obfuscating a real object), the framework will set a transparency to the virtual object to avoid the user's collision with the real object. The policy framework manages also non-visual outputs such as audio and haptic. The output framework in XROS also manages the priority to display output (visual, audio, haptic) when several XR applications are used simultaneously. 









